ControlVideo: Training-free Controllable Text-to-Video Generation

Text-driven diffusion models have unlocked unprecedented abilities in image generation, whereas their video counterpart still lags behind due to the excessive training cost of temporal modeling. Besides the training burden, the generated videos also suffer from appearance inconsistency and structural flickers, especially in long video synthesis. To address these challenges, we design a \emph{training-free} framework called \textbf{ControlVideo} to enable natural and efficient text-to-video generation. ControlVideo, adapted from ControlNet, leverages coarsely structural consistency from input motion sequences, and introduces three modules to improve video generation. Firstly, to ensure appearance coherence between frames, ControlVideo adds fully cross-frame interaction in self-attention modules. Secondly, to mitigate the flicker effect, it introduces an interleaved-frame smoother that employs frame interpolation on alternated frames. Finally, to produce long videos efficiently, it utilizes a hierarchical sampler that separately synthesizes each short clip with holistic coherency. Empowered with these modules, ControlVideo outperforms the state-of-the-arts on extensive motion-prompt pairs quantitatively and qualitatively. Notably, thanks to the efficient designs, it generates both short and long videos within several minutes using one NVIDIA 2080Ti. Code is available at https://github.com/YBYBZhang/ControlVideo.

==> figText/supp_comare.tex <==
\begin{figure}[t]
%   \vspace{-1em}
  \begin{center}
  \includegraphics[width=.99\linewidth]{figures/supp_com_canny.pdf}
  \end{center}
  \vspace{-1mm}
  \caption{
  \textbf{More qualitative comparisons conditioned on canny edges.}
  \textbf{Results best seen at 500\% zoom.}
  }
    \label{fig:supp_com_canny}
  \vspace{-1mm}
\end{figure}

\begin{figure}[t]
%   \vspace{-1em}
  \begin{center}
  \includegraphics[width=.99\linewidth]{figures/supp_com_depth.pdf}
  \end{center}
  \vspace{-1mm}
  \caption{
  \textbf{More qualitative comparisons conditioned on depth maps.}
  \textbf{Results best seen at 500\% zoom.}
  }
    \label{fig:supp_com_depth}
  \vspace{-1mm}
\end{figure}

\begin{figure}[t]
%   \vspace{-1em}
  \begin{center}
  \includegraphics[width=.99\linewidth]{figures/supp_com_pose.pdf}
  \end{center}
  \vspace{-1mm}
  \caption{
  \textbf{More qualitative comparisons conditioned on human poses.}
  \textbf{Results best seen at 500\% zoom.}
  }
    \label{fig:supp_com_pose}
  \vspace{-1mm}
\end{figure}

==> figText/supp_smoother.tex <==
\begin{figure}[t]
%   \vspace{-1em}
  \begin{center}
  \includegraphics[width=.95\linewidth]{figures/ab_smoother_time.pdf}
  \end{center}
  \vspace{-1mm}
  \caption{
  \textbf{.}
  \textbf{Results best seen at 500\% zoom.}
  }
    \label{fig:ab_smoother_time}
  \vspace{-1mm}
\end{figure}

\begin{figure}[t]
%   \vspace{-1em}
  \begin{center}
  \includegraphics[width=.95\linewidth]{figures/ab_smoother_number.pdf}
  \end{center}
  \vspace{-1mm}
  \caption{
  \textbf{.}
  \textbf{Results best seen at 500\% zoom.}
  }
    \label{fig:ab_smoother_number}
  \vspace{-1mm}
\end{figure}

==> figText/supp_visualize.tex <==
\begin{figure}[t]
%   \vspace{-1em}
  \begin{center}
  \includegraphics[width=.95\linewidth]{figures/supp_canny.pdf}
  \end{center}
  \vspace{-1mm}
  \caption{
  \textbf{More video visualizations conditioned on canny edges.}
  \textbf{Results best seen at 500\% zoom.}
  }
    \label{fig:supp_canny}
  \vspace{-1mm}
\end{figure}

\begin{figure}[t]
%   \vspace{-1em}
  \begin{center}
  \includegraphics[width=.95\linewidth]{figures/supp_depth.pdf}
  \end{center}
  \vspace{-1mm}
  \caption{
  \textbf{More video visualizations conditioned on depth maps.}
  \textbf{Results best seen at 500\% zoom.}
  }
    \label{fig:supp_depth}
  \vspace{-1mm}
\end{figure}

\begin{figure}[t]
%   \vspace{-1em}
  \begin{center}
  \includegraphics[width=.95\linewidth]{figures/supp_pose.pdf}
  \end{center}
  \vspace{-1mm}
  \caption{
  \textbf{More video visualizations conditioned on human poses.}
  \textbf{Results best seen at 500\% zoom.}
  }
    \label{fig:supp_pose}
  \vspace{-1mm}
\end{figure}

\begin{figure}[t]
%   \vspace{-1em}
  \begin{center}
  \includegraphics[width=.9\linewidth]{figures/supp_long.pdf}
  \end{center}
  \vspace{-1mm}
  \caption{
  \textbf{Additional long video visualization.}
  \textbf{Results best seen at 500\% zoom.}
  }
    \label{fig:supp_long}
  \vspace{-1mm}
\end{figure}

\begin{figure}[t]
%   \vspace{-1em}
  \begin{center}
  \includegraphics[width=.99\linewidth]{figures/supp_limitation.pdf}
  \end{center}
  \vspace{-1mm}
  \caption{\textbf{Limitation visualizations.}
  ControlVideo struggles with producing videos beyond input motion sequences.
  The motion of text prompt \texttt{Iron man \textcolor{red}{runs} on the street} does not align with the given sequential poses of \texttt{Michael Jackson's moonwalk}, which degrades the video quality and consistency.
  }
    \label{fig:supp_limitation}
  \vspace{-1mm}
\end{figure}

==> figText/user_instruction.tex <==
\begin{figure}[t!]
   \begin{center}
   \includegraphics[width=.85\linewidth]{figures/user_example.pdf}
   \end{center}
  \vspace{-2mm}
   \caption{
   \textbf{The instruction of user study.}
   A user study sample consists of a text prompt, structure sequence, and synthesized videos from two different methods (in random order).
   The raters are asked to answer the above three questions for each sample.
    }
    \label{fig:user_instruction}
    \vspace{-1em}
\end{figure}

==> table/supp_data.tex <==
\begin{table}[t]
\caption{
    \textbf{Names and captions of selected videos from DAVIS dataset.}}
    \vspace{2mm}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{lc}
    \toprule
         \makecell{Video Name} & \makecell{Source Caption} \\
         % \Xhline{\arrayrulewidth}
         \midrule
         blackswan &{a black swan moving on the lake} \\
         boat &{a boat moves in the river} \\
         breakdance-flare &{a man dances on the road} \\
         bus &{a bus moves on the street} \\
         camel &{a camel walks on the desert} \\
         car-roundabout &{a jeep turns on a road} \\
         car-shadow &{a car moves to a building} \\
         car-turn &{a jeep on a forest road} \\
         cows &{a cow walks on the grass} \\
         dog &{a dog walks on the ground} \\
         elephant &{an elephant walks on the ground} \\
         flamingo &{a flamingo wanders in the water} \\
         gold-fish &{golden fishers swim in the water} \\
         hike &{a man hikes on a mountain} \\
         hockey &{a player is playing hockey on the ground} \\
         kite-surf &{a man is surfing on the sea} \\
         lab-coat &{three women stands on the lawn} \\
         longboard &{a man is playing   skateboard on the alley} \\
         mallard-water &{a mallard swims on the water} \\
         mbike-trick &{a man riding motorbike} \\
         rhino &{a rhino walks on the rocks} \\
         surf &{a sailing boat moves on the sea} \\
         swing &{a girl is playing on the swings} \\
         tennis &{a man is playing tennis} \\
         walking &{a selfie of walking man} \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-2mm}
    \label{tab:supp_data}
\end{table}
